Accelerated Riemannian Optimization: Handling Constraints with a Prox to Bound Geometric Penalties

We propose a globally-accelerated, first-order method for the optimization of smooth and (strongly or not) geodesically-convex functions in a wide class of Hadamard manifolds. We achieve the same convergence rates as Nesterov's accelerated gradient descent, up to a multiplicative geometric penalty and log factors. Crucially, we can enforce our method to stay within a compact set we define. Prior fully accelerated works \emph{resort to assuming} that the iterates of their algorithms stay in some pre-specified compact set, except for two previous methods of limited applicability. For our manifolds, this solves the open question in [KY22] about obtaining global general acceleration without iterates assumptively staying in the feasible set. In our solution, we design an accelerated Riemannian inexact proximal point algorithm, which is a result that was unknown even with exact access to the proximal operator, and is of independent interest. For smooth functions, we show we can implement the prox step inexactly with first-order methods in Riemannian balls of certain diameter that is enough for global accelerated optimization.

==> definitions.tex <==

\usepackage{xparse}
\usepackage{xargs}

\makeatletter 
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\usepackage{etoolbox}
\robustify{\hyperlink}

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} 

\makeatother




\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{\newtarget{proof:#1}}


\usepackage[bb=boondox]{mathalpha} 

\newcommand{\zeros}{\mathbb{0}} 

\newcommand{\GD}{\newlink{def:acronym_gradient_descent}{GD}}
\newcommand{\AGD}{\newlink{def:acronym_accelerated_gradient_descent}{AGD}}
\newcommand{\RGD}{\newlink{def:acronym_riemannian_gradient_descent}{RGD}}
\newcommand{\MD}{\newlink{def:acronym_mirror_descent}{MD}}

\newcommand{\bigoast}[1]{\newlink{def:big_o_ast}{O^\ast}( #1 )}
\newcommand{\bigoastl}[1]{\newlink{def:big_o_ast}{O^\ast}\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}

\newcommand{\riemaconsc}{\newlink{def:Riemacon_SC}{RiemaconSC}}
\newcommand{\riemacon}{\newlink{def:Riemacon}{Riemacon}}


\newcommand\B{\mathcal{B}}

\let\oldmu\mu
\renewcommand\mu{\newlink{def:strong_g_convexity_of_F}{\oldmu}}


\let\oldPii\Pi
\newcommand\Pii[1]{\newlink{def:euclidean_projection}{\oldPii_{#1}}}

\let\olddelta\delta
\renewcommand\delta[1]{\newlink{def:delta}{\olddelta_{#1}}}
\newcommand\deltad{\newlink{def:delta_without_subindex_which_means_zeta_D}{\bar{\olddelta}}}
\newcommand\deltar{\newlink{def:delta_without_subindex_which_means_zeta_RR}{\olddelta}}
\let\oldzeta\zeta
\renewcommand\zeta[1]{\newlink{def:zeta}{\oldzeta_{#1}}}
\newcommand\zetasq[1]{\newlink{def:zeta}{\oldzeta_{#1}^2}}
\newcommand\zetad{\newlink{def:zeta_without_subindex_which_means_zeta_D}{\bar{\oldzeta}}}
\newcommand\zetar{\newlink{def:zeta_without_subindex_which_means_zeta_RR}{\oldzeta}}


\newcommandx*\kmin[1][1=, usedefault]{\newlink{def:minimum_sectional_curvature}{\kappa_{\min}^{#1}}}
\newcommandx*\kmax[1][1=, usedefault]{\newlink{def:maximum_sectional_curvature}{\kappa_{\max}^{#1}}}


\renewcommand\M{\newlink{def:M_manifold}{\mathcal{M}}}
\newcommand\MOnly{\mathcal{M}}
\renewcommand\H{\newlink{def:H_hadamard}{\mathcal{H}}}
\newcommand\NN{\newlink{def:N_open_set_in_manifold}{\mathcal{N}}}
\newcommand{\X}{\newlink{def:geodesically_convex_feasible_region}{\mathcal{X}}}
\renewcommand{\D}{\newlink{def:diameter_of_geodesically_convex_feasible_region}{D}}
\renewcommand\d{\mathrm{d}}

\newcommand{\Tri}{\mathcal{T}}
\newcommand\MEucl{\newlink{def:M_Euclidean}{M}}


\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}
\newcommand{\epsilonp}{\newlink{def:accuracy_epsilon_prime_in_ball_subproblem}{\oldepsilon'}}
\newcommandx*\hatepsilon[1][1=i, usedefault]{\newlink{def:accuracy_of_binary_search}{\hat{\oldepsilon}_{#1}}}


\newcommandx{\sigmak}[1][1=k, usedefault]{\newlink{def:accuracy_of_prox_subproblems}{\sigma_{#1}}}

\newcommand{\TT}{\newlink{def:total_number_of_iterations_of_instanced_algorithm}{T}}

\let\oldGamma\Gamma
\renewcommand{\Gamma}[2]{\newlink{def:parallel_transport}{\oldGamma_{#1}^{#2}}}

\let\oldlambda\lambda
\renewcommand{\lambda}{\newlink{def:implicit_GD_learning_rate_lambda}{\oldlambda}}

\let\xiOnly\xi
\renewcommand{\xi}{\newlink{def:extra_geom_penalty_xi}{\xiOnly}}



\newcommandx*\errork[1][1=k, usedefault]{\newlink{def:error_k_from_approximating_grad}{\oldepsilon_{#1}}}

\newcommandx*\proj[1][1=\X, usedefault]{\newlink{def:projection_operator}{\mathcal{P}_{#1}}}

\newcommand\expon[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Exp}_{#1}}} 
\newcommand\exponinv[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Log}_{#1}}} 


\newcommand{\n}{\newlink{def:dimension}{n}} 
\newcommand{\Lips}{\newlink{def:Lipschitz_constant}{L_{\mathtt{p}}}} 
\newcommand{\Ltildegeneric}{\newlink{def:generic_smoothness_in_euclidean_case}{\tilde{L}}} 
\newcommand{\Ltilde}{\newlink{def:smoothness_tilde_i_e_euclidean_coming_from_riemannian}{\tilde{L}}} 

\let\strikedL\L
\renewcommand{\L}{\newlink{def:riemannian_smoothness_of_F}{L}} 

\renewcommand{\time}{\newlink{def:time_alg_of_strongly_convex_for_reduction}{\operatorname{Time}}}
\newcommand{\timens}{\newlink{def:time_alg_of_just_convex_for_reduction}{\operatorname{Time}_{\operatorname{ns}}}}
\newcommand{\Alg}{\newlink{def:alg_of_strongly_convex_for_reduction}{\mathcal{A}}}
\newcommand{\Algns}{\newlink{def:alg_of_just_convex_for_reduction}{\mathcal{A}_{\operatorname{ns}}}}
\newcommand{\Q}{\newlink{def:convex_set_of_tilted_convex_thm}{Q}}


\newcommand{\dist}{\newlink{def:distance}{d}}

\let\oldPhi\Phi
\renewcommand{\Phi}{\newlink{def:squared_distance_function_div_by_2}{\oldPhi}}

\newcommandx*{\psik}[1][1=k, usedefault]{\newlink{def:function_for_Lyapunov_analysis}{\psi_{#1}}}

\newcommand{\astfenchel}{\newlink{def:asterisk_of_fenchel_dual}{\ast}}
\let\oldPi\Pi
\renewcommand{\Pi}{\newlink{def:euclidean_projection}{\oldPi}}

\renewcommand{\K}{\newlink{def:curvature}{K}} 
\newcommand{\deltaAux}{\newlink{def:auxiliary_angle_delta}{\delta}} 
\newcommand{\deltatildeAux}{\newlink{def:auxiliary_angle_delta}{\tilde{\delta}}} 
\newcommand{\deltapAux}{\newlink{def:auxiliary_delta_prime}{\delta'}} 
\newcommand{\deltaptildeAux}{\newlink{def:auxiliary_delta_prime}{\tilde{\delta}'}} 
\newcommand{\deltaastAux}{\newlink{def:auxiliary_delta_ast}{\delta^\ast}} 
\newcommand{\deltaasttildeAux}{\newlink{def:auxiliary_delta_ast}{\tilde{\delta}^\ast}}


\newcommandx*\sk[2][1= , 2= , usedefault]{\newlink{def:special_sine}{\operatorname{S}_{\K}^{#2}}( #1 )}
\newcommandx*\ck[2][1= , 2= , usedefault]{\newlink{def:special_cosine}{\operatorname{C}_{\K}^{#2}}( #1 )}
\newcommandx*\cotk[2][1= , 2= , usedefault]{\newlink{def:special_cotangent}{\operatorname{cot}_{\K}^{#2}}( #1 )}


\newcommand{\distorp}{\newlink{def:distortion_K_pos}{\mathcal{K}_R^+}}
\newcommand{\distorn}{\newlink{def:distortion_K_neg}{\mathcal{K}_R^-}}



\newcommand{\affLowerBound}{\newlink{def:affine_lower_bound}{\ell}}
\newcommand\lambdanot[1]{\newlink{def:lambda_superscript_notation}{#1}}

\newcommandx*\Ei[1][1=i, usedefault]{\newlink{def:discretization_error}{E_{#1}}}

\newcommandx*\Di[1][1=i, usedefault]{\newlink{def:gap_for_reduction_tost_g_convex}{D_{#1}}}

\newcommandx*\FReg[1][1=i, usedefault]{\newlink{def:regularized_F_for_reduction}{F^{(#1)}}}

\newcommandx*\Deltak[2][1=k, 2=, usedefault]{\newlink{def:loss_factor_in_Lyapunov}{\Delta_{#1}^{#2}}}

\newcommand\f{\newlink{def:riemannian_function_f}{f}}
\newcommand\ftilted{\newlink{def:tilted_convex_function_generic_euclidean}{f}}

\newcommandx*\RInit[1][1=, usedefault]{\newlink{def:initial_distance_for_X}{\bar{R}^{#1}}}
\newcommand\RR{\newlink{def:distance_or_bound_to_global_minimizer}{R}}


\newcommand\Rp{\newlink{def:R_plus}{\R^{+}}}



\newcommand\ball{\newlink{def:closed_ball}{\bar{B}}}

\newcommandx*\hatgamma[1][1=i, usedefault]{\newlink{def:tilted_parameter_at_iteration_i}{\hat{\gamma}_{#1}}}
\newcommandx*\Gammahat[2][1=i, 2= , usedefault]{\newlink{def:function_for_tilted_parameter}{\hat{\Gamma}_{#1}^{#2}}}

\newcommandx*\Gt[1][1=t, usedefault]{\newlink{def:differentiable_gap_bound}{G_{#1}}}
\newcommandx*\Lt[1][1=t, usedefault]{\newlink{def:differentiable_lower_bound}{L_{#1}}}
\newcommandx*\Ut[1][1=t, usedefault]{\newlink{def:differentiable_upper_bound}{U_{#1}}}
\newcommandx*\Gbinsearch[1][1=i, usedefault]{\newlink{def:G_binary_search}{\mathcal{G}_{#1}}}

\newcommandx*\Ak[2][1=k, 2=, usedefault]{\newlink{def:integral_of_steps}{A_{#1}^{#2}}}
\newcommandx*\ak[2][1=k, 2=, usedefault]{\newlink{def:discrete_step}{a_{#1}^{#2}}}
\newcommandx*\Akp[2][1=k, 2=, usedefault]{\newlink{def:integral_of_steps}{A_{#1}'^{#2}}}
\newcommandx*\akp[2][1=k, 2=, usedefault]{\newlink{def:discrete_step}{a_{#1}'^{#2}}}
\newcommandx*\ey[1][1=k, usedefault]{\newlink{def:discrete_step}{e_{#1}^y}}
\newcommandx*\ex[1][1=k, usedefault]{\newlink{def:discrete_step}{e_{#1}^x}}

\newcommandx*\alphat[1][1=, usedefault]{\newlink{def:step_function_alpha}{\alpha_{#1}}}

\newcommand\Tansp[1]{\newlink{def:tangent_space}{T_{#1}}}


\newcommand\notilde{\noop}

\newcommandx*\etak[2][1=k,2=, usedefault]{\newlink{def:MD_step_length}{\eta_{#1}^{#2}}}
\newcommandx*\tauk[1][1=k, usedefault]{\newlink{def:aux_tau_k}{\tau_{#1}}}

\newcommandx*\hk[1][1=k, usedefault]{\newlink{def:proximal_objective}{h_{#1}}}

\newcommandx*\yk[1][1=k, usedefault]{\newlink{def:iterate_y}{y_{#1}}}
\newcommandx*\ykast[1][1=k, usedefault]{\newlink{def:optimal_proximal_operator}{y_{#1}^{\ast}}}
\newcommandx*\xk[2][1=k,2=, usedefault]{\newlink{def:iterate_x}{x_{#1}^{#2}}}
\newcommandx*\xkp[2][1=k,2=, usedefault]{\newlink{def:iterate_xp}{x_{#1}'^{#2}}}
\newcommandx*\zy[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_y}{z_{#1}^{y_{#2}}}}

\newcommandx*\zybar[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_y_bar}{\bar{z}_{#1}^{y_{#2}}}}
\newcommandx*\zx[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_x}{z_{#1}^{x_{#2}}}}
\newcommand\xInit{\newlink{def:initial_point}{x_0}}
\newcommand\xast{\newlink{def:optimizer_at_X}{\bar{x}^\ast}}
\newcommand\xastg{\newlink{def:global_optimizer}{x^\ast}}

\newcommandx*\vkx[1][1=k, usedefault]{\newlink{def:v_k_sup_x}{v_{#1}^{x}}}
\newcommandx*\vtkx[1][1=k, usedefault]{\newlink{def:v_tilde_k_sup_x}{\tilde{v}_{#1}^{x}}}
\newcommandx*\vtky[1][1=k, usedefault]{\newlink{def:v_tilde_k_sup_y}{\tilde{v}_{#1}^{y}}}

\newcommandx*\lossk[2][1=k, 2= , usedefault]{\newlink{def:losses_primal}{\ell^{(#1)}_{#2}}}
\newcommand\Hess{\operatorname{Hess}}


\newcommand\prox[1]{\newlink{def:prox}{\operatorname{prox}(#1)}}
\renewcommand\W{\mathcal{W}} 
\renewcommand\c{\newlink{def:constants_in_martinez2020global}{c}}

\newcommand\curvtensor{\newlink{def:curvature_tensor}{\mathfrak{R}}}
\newcommand\indicator[1]{\newlink{def:indicator_function}{I_{#1}}}

